A Preliminary Study of RAG for Taiwanese Historical Archives

Retrieval-Augmented Generation (RAG) has emerged as a promising approach for knowledge-intensive tasks. However, few studies have examined RAG for Taiwanese Historical Archives. In this paper, we present an initial study of a RAG pipeline applied to two historical Traditional Chinese datasets, Fort Zeelandia and the Taiwan Provincial Council Gazette, along with their corresponding open-ended query sets. We systematically investigate the effects of query characteristics and metadata integration strategies on retrieval quality, answer generation, and the performance of the overall system. The results show that early-stage metadata integration enhances both retrieval and answer accuracy while also revealing persistent challenges for RAG systems, including hallucinations during generation and difficulties in handling temporal or multi-hop historical queries.

==> ROCLING2025/figure/fortzeelandia.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[height=5cm, width=\linewidth]{ROCLING2025/static/fort_question.png}
    \caption{Question types in the Fort Zeelandia dataset. Left: Distribution of each entity focus. Note that questions may focus on multiple entities. Right: Distribution of entity focus across different question complexities.}
    \label{fig:fortzeelandia_question_distribution}
\end{figure*}


==> ROCLING2025/section/Discussion.tex <==
\section{Discussion}
Our results show that early-stage integration with document-level metadata leads to the greatest improvements in both retrieval and generation performance. However, key challenges remain: the system struggles with hallucination during generation. As shown in Table \ref{tab:rag_score_gold}, providing gold passages enhances performance compared to the best-performing question and method types on the two datasets, implying that retrieval is the primary bottleneck. Yet even with golden passage provided, the model sometimes incorporates irrelevant information, highlighting persistent challenges in accurate information integration during generation.

==> ROCLING2025/table/exp_table.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Integration Stage} & \textbf{Metadata Type} & \textbf{Retriever} & \textbf{Recall@5} \\
\midrule
\multirow{4}{*}{Baseline} & \multirow{4}{*}{None} & BM25 & 0.2143 \\
 & & BGE-M3 Sparse & 0.1786 \\
 & & BGE-M3 Dense & 0.0893 \\
 & & Hybrid & 0.1429 \\
\midrule
\multirow{12}{*}{Metadata-Augmented Retrieval} & \multirow{4}{*}{Time/Event} & BM25 & 0.2679 \\
 & & BGE-M3 Sparse & 0.2500 \\
 & & BGE-M3 Dense & 0.2142 \\
 & & Hybrid & 0.2321 \\
\cline{2-4}
 & \multirow{4}{*}{Person/Organization} & BM25 & 0.2679 \\
 & & BGE-M3 Sparse & 0.2679 \\
 & & BGE-M3 Dense & 0.1429 \\
 & & Hybrid & 0.2321 \\
\cline{2-4}
 & \multirow{4}{*}{Document/Content} & BM25 & 0.4821 \\
 & & BGE-M3 Sparse & 0.5000 \\
 & & BGE-M3 Dense & 0.3571 \\
 & & Hybrid & 0.5000 \\
\midrule
\multirow{12}{*}{Metadata-Guided Reranking} & \multirow{4}{*}{Time/Event} & BM25 & 0.0893 \\
 & & BGE-M3 Sparse & 0.1250 \\
 & & BGE-M3 Dense & 0.1250 \\
 & & Hybrid & 0.1429 \\
\cline{2-4}
 & \multirow{4}{*}{Person/Organization} & BM25 & 0.1071 \\
 & & BGE-M3 Sparse & 0.1250 \\
 & & BGE-M3 Dense & 0.1250 \\
 & & Hybrid & 0.1429 \\
\cline{2-4}
 & \multirow{4}{*}{Document/Content} & BM25 & 0.3929 \\
 & & BGE-M3 Sparse & 0.4286 \\
 & & BGE-M3 Dense & 0.3393 \\
 & & Hybrid & 0.4464 \\
\midrule
\multirow{12}{*}{Metadata-Augmented Reranking} & \multirow{4}{*}{Time/Event} & BM25 & 0.3393 \\
 & & BGE-M3 Sparse & 0.0893 \\
 & & BGE-M3 Dense & 0.1071 \\
 & & Hybrid & 0.1429 \\
\cline{2-4}
 & \multirow{4}{*}{Person/Organization} & BM25 & 0.2321 \\
 & & BGE-M3 Sparse & 0.1071 \\
 & & BGE-M3 Dense & 0.1607 \\
 & & Hybrid & 0.1607 \\
\cline{2-4}
 & \multirow{4}{*}{Document/Content} & BM25 & 0.3393 \\
 & & BGE-M3 Sparse & 0.3929 \\
 & & BGE-M3 Dense & 0.3036 \\
 & & Hybrid & 0.4286 \\
\bottomrule
\end{tabular}
\caption{Retrieval Performance Across Metadata Integration Strategies}
\end{table*}


==> ROCLING2025/table/fort_complexity_focus.tex <==
\begin{table}[h]
    \centering
    \begin{minipage}[t]{0.45\linewidth}
        \centering
        \caption{Fort Zeelandia Question Complexity}
        \begin{tabular}{lc}
            \toprule
            \textbf{Complexity} & \textbf{Count} \\
            \midrule
            Single-hop & 100 \\
            Multi-hop & 73 \\
            \bottomrule
        \end{tabular}
    \end{minipage}
    \hspace{0.05\linewidth} % Horizontal space between the tables
    \begin{minipage}[t]{0.45\linewidth}
        \centering
        \caption{Fort Zeelandia Question Entity Focus}
        \begin{tabular}{lc}
            \toprule
            \textbf{Entity} & \textbf{Count} \\
            \midrule
            People & 44 \\
            Event  & 80 \\
            Item   & 21 \\
            Place  & 44 \\
            Time   & 41 \\
            \bottomrule
        \end{tabular}
    \end{minipage}
\end{table}


==> ROCLING2025/table/fort_entity_focus_exp.tex <==
\begin{table}[H]
    \centering
    \caption{Average Recall@5 per Entity Focus across Different Retrievers}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Entity} & \textbf{Sparse} & \textbf{Dense} & \textbf{Hybrid} \\
        \midrule
        People        & 0.5228 & 0.5011 & 0.5543 \\
        Event         & 0.4634 & 0.4618 & 0.5504 \\
        Time          & 0.4348 & 0.3478 & 0.4348 \\
        Place         & 0.5262 & 0.4865 & 0.4865 \\
        Item          & 0.4375 & 0.6250 & 0.5000 \\
        Multi-entity  & 0.3536 & 0.2398 & 0.3350 \\
        \bottomrule
    \end{tabular}
\end{table}


==> ROCLING2025/table/golden_passage.tex <==
\begin{table*}[ht]
\small
\centering
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccc}
\toprule
\textbf{Method} & \textbf{Dataset} & \textbf{Gold} & \textbf{Relevant} & \textbf{Hallucinated} \\
\midrule
Gold Passages Provided & Fort Zeelandia & 4.4104 & 0.2312 & -0.2601 \\
Event-type Questions using Baseline Retrieval & Fort Zeelandia & 3.4600 & 1.2200 & -0.5800 \\
Gold Passages Provided & TPCG & 3.6964 & 0.0179 & -0.0714 \\
Metadata-Augmented Retrieval with Document Type & TPCG & 2.1429 & 1.2500 & -0.3214 \\
\bottomrule
\end{tabular*}
\caption{RAG evaluation comparing performance with gold passages against the best-performing methods on two datasets.}
\label{tab:rag_score_gold}
\end{table*}
